Do Large Language Models Pay Similar Attention Like Human Programmers When Generating Code?

Large Language Models (LLMs) have recently been widely used for code generation. Due to the complexity and opacity of LLMs, little is known about how these models generate code. We made the first attempt to bridge this knowledge gap by investigating whether LLMs attend to the same parts of a task description as human programmers during code generation. An analysis of six LLMs, including GPT-4, on two popular code generation benchmarks revealed a consistent misalignment between LLMs' and programmers' attention. We manually analyzed 211 incorrect code snippets and found five attention patterns that can be used to explain many code generation errors. Finally, a user study showed that model attention computed by a perturbation-based method is often favored by human programmers. Our findings highlight the need for human-aligned LLMs for better interpretability and programmer trust.

==> gradient_table.tex <==
\hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{12}{c|}{\textbf{Input$\times$Gradient\_reading}}                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{12}{c|}{\textbf{Input$\times$Gradient\_coding}}                                                                                                                                                                                                                                                                                                                                                       \\ \cline{2-25} 
                                 & \multicolumn{4}{c|}{\textbf{Top 5}}                                                                                                  & \multicolumn{4}{c|}{\textbf{Top 10}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Top 20}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Top 5}}                                                                                                  & \multicolumn{4}{c|}{\textbf{Top 10}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Top 20}}                                                                                                 \\ \cline{2-25} 
                                 & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} \\ \hline
\textbf{Incoder}                 & 62.4\%                         & 38.4\%                         & 47.6\%                          & \multicolumn{1}{r|}{-0.21}       & 69.7\%                         & 67.1\%                         & 68.4\%                          & \multicolumn{1}{r|}{-0.01}       & 71.7\%                         & 94.4\%                         & 81.5\%                          & 0.02                             & 55.5\%                         & 32.1\%                         & 40.7\%                          & \multicolumn{1}{r|}{-0.3}        & 66.6\%                         & 61.7\%                         & 64.1\%                          & \multicolumn{1}{r|}{-0.06}       & 70.5\%                         & 93.3\%                         & 80.4\%                          & 0.02                             \\ \cline{1-1}
\textbf{CodeGen}                 & 59.9\%                         & 37.6\%                         & 46.2\%                          & \multicolumn{1}{r|}{-0.23}       & 68.2\%                         & 65.6\%                         & 66.9\%                          & \multicolumn{1}{r|}{-0.03}       & 70.8\%                         & 93.3\%                         & 80.5\%                          & 0.02                             & 51.7\%                         & 32.1\%                         & 39.6\%                          & \multicolumn{1}{r|}{-0.32}       & 63.9\%                         & 62.7\%                         & 63.3\%                          & \multicolumn{1}{r|}{-0.09}       & 68.3\%                         & 93.8\%                         & 79.1\%                          & -0.02                            \\ \cline{1-1}
\textbf{CodeParrot}              & 42.2\%                         & 27.5\%                         & 33.3\%                          & \multicolumn{1}{r|}{-0.18}       & 47.8\%                         & 55.3\%                         & 51.3\%                          & \multicolumn{1}{r|}{-0.13}       & 53.6\%                         & 90.7\%                         & 67.4\%                          & -0.12                            & 71.2\%                         & 46.7\%                         & 56.4\%                          & \multicolumn{1}{r|}{0.17}        & 65.8\%                         & 71.5\%                         & 68.5\%                          & \multicolumn{1}{r|}{0.22}        & 60.2\%                         & 94.4\%                         & 73.5\%                          & 0.01                             \\ \cline{1-1}
\textbf{GPT-J-6B}                & 46.2\%                         & 30.1\%                         & 36.4\%                          & \multicolumn{1}{r|}{-0.11}       & 49.0\%                         & 57.3\%                         & 52.8\%                          & \multicolumn{1}{r|}{-0.07}       & 53.1\%                         & 91.4\%                         & 67.2\%                          & -0.1                             & 73.3\%                         & 48.2\%                         & 58.2\%                          & \multicolumn{1}{r|}{0.21}        & 66.0\%                         & 72.2\%                         & 68.9\%                          & \multicolumn{1}{r|}{0.23}        & 60.5\%                         & 94.5\%                         & 73.8\%                          & 0.03                             \\ \cline{1-1}
\textbf{PolyCoder}               & 70.3\%                         & 45.4\%                         & 55.2\%                          & \multicolumn{1}{r|}{0.14}        & 67.2\%                         & 73.6\%                         & 70.2\%                          & \multicolumn{1}{r|}{0.24}        & 60.9\%                         & 94.6\%                         & 74.1\%                          & 0                                & 77.7\%                         & 51.6\%                         & 62.0\%                          & \multicolumn{1}{r|}{0.27}        & 71.9\%                         & 78.4\%                         & 75.0\%                          & \multicolumn{1}{r|}{0.37}        & 62.0\%                         & 95.3\%                         & 75.1\%                          & 0.06                             \\ \hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{12}{c|}{\textbf{Saliency\_reading}}                                                                                                                                                                                                                                                                                                                                                                   & \multicolumn{12}{c|}{\textbf{Saliency\_coding}}                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-25} 
                                 & \multicolumn{4}{c|}{\textbf{Top 5}}                                                                                                  & \multicolumn{4}{c|}{\textbf{Top 10}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Top 20}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Top 5}}                                                                                                  & \multicolumn{4}{c|}{\textbf{Top 10}}                                                                                                 & \multicolumn{4}{c|}{\textbf{Top 20}}                                                                                                 \\ \cline{2-25} 
                                 & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} & \multicolumn{1}{c}{\textbf{P}} & \multicolumn{1}{c}{\textbf{R}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{KA}} \\ \hline
\textbf{Incoder}                 & 68.2\%                         & 43.8\%                         & 53.4\%                          & \multicolumn{1}{r|}{0.11}        & 65.1\%                         & 71.2\%                         & 68.0\%                          & \multicolumn{1}{r|}{0.19}        & 60.3\%                         & 94.1\%                         & 73.5\%                          & -0.01                            & 77.8\%                         & 51.1\%                         & 61.7\%                          & \multicolumn{1}{r|}{0.26}        & 71.6\%                         & 77.4\%                         & 74.4\%                          & \multicolumn{1}{r|}{0.35}        & 62.2\%                         & 95.2\%                         & 75.3\%                          & 0.06                             \\ \cline{1-1}
\textbf{CodeGen}                 & 49.2\%                         & 33.0\%                         & 39.5\%                          & \multicolumn{1}{r|}{-0.1}        & 53.6\%                         & 60.8\%                         & 57.0\%                          & \multicolumn{1}{r|}{-0.02}       & 55.9\%                         & 91.7\%                         & 69.5\%                          & -0.07                            & 59.2\%                         & 40.4\%                         & 48.0\%                          & \multicolumn{1}{r|}{0.04}        & 58.8\%                         & 66.1\%                         & 62.2\%                          & \multicolumn{1}{r|}{0.1}         & 57.1\%                         & 92.6\%                         & 70.6\%                          & -0.03                            \\ \cline{1-1}
\textbf{CodeParrot}              & 48.2\%                         & 30.2\%                         & 37.2\%                          & \multicolumn{1}{r|}{-0.14}       & 55.2\%                         & 62.5\%                         & 58.6\%                          & \multicolumn{1}{r|}{0}           & 56.8\%                         & 92.5\%                         & 70.4\%                          & -0.06                            & 62.2\%                         & 40.5\%                         & 49.0\%                          & \multicolumn{1}{r|}{0.06}        & 59.9\%                         & 65.7\%                         & 62.7\%                          & \multicolumn{1}{r|}{0.11}        & 58.1\%                         & 92.5\%                         & 71.4\%                          & -0.01                            \\ \cline{1-1}
\textbf{GPT-J-6B}                & 50.7\%                         & 32.7\%                         & 39.7\%                          & \multicolumn{1}{r|}{-0.11}       & 55.8\%                         & 62.4\%                         & 58.9\%                          & \multicolumn{1}{r|}{-0.01}       & 57.7\%                         & 92.5\%                         & 71.0\%                          & -0.06                            & 55.0\%                         & 36.1\%                         & 43.6\%                          & \multicolumn{1}{r|}{-0.03}       & 57.6\%                         & 64.6\%                         & 60.9\%                          & \multicolumn{1}{r|}{0.07}        & 57.2\%                         & 93.9\%                         & 71.1\%                          & -0.03                            \\ \cline{1-1}
\textbf{PolyCoder}               & 51.3\%                         & 32.7\%                         & 39.9\%                          & \multicolumn{1}{r|}{-0.11}       & 55.8\%                         & 62.1\%                         & 58.8\%                          & \multicolumn{1}{r|}{-0.01}       & 58.0\%                         & 93.2\%                         & 71.5\%                          & -0.06                            & 54.0\%                         & 35.9\%                         & 43.1\%                          & \multicolumn{1}{r|}{-0.05}       & 57.3\%                         & 64.0\%                         & 60.5\%                          & \multicolumn{1}{r|}{0.06}        & 57.5\%                         & 93.7\%                         & 71.3\%                          & -0.03                            \\ \hline
\end{tabular}
